On Achievable Rates Over Noisy Nanopore Channels

In this paper, we consider a recent channel model of a nanopore sequencer proposed by McBain, Viterbo, and Saunderson (2024), termed the noisy nanopore channel (NNC). In essence, an NNC is a duplication channel with structured, Markov inputs, that is corrupted by memoryless noise. We first discuss a (tight) lower bound on the capacity of the NNC in the absence of random noise. Next, we present lower and upper bounds on the channel capacity of general noisy nanopore channels. We then consider two interesting regimes of operation of an NNC: first, where the memory of the input process is large and the random noise introduces erasures, and second, where the rate of measurements of the electric current (also called the sampling rate) is high. For these regimes, we show that it is possible to achieve information rates close to the noise-free capacity, using low-complexity encoding and decoding schemes. In particular, our decoder for the regime of high sampling rates makes use of a change-point detection procedure -- a subroutine of immediate relevance for practitioners.

==> convergence.tex <==
\label{sec:convergence}
In this section, we prove Theorem \ref{thm:conv} for the mutual information (or information rate) $I^{(d)}$ of a DMC $W$ with an aribitrary distribution $P_X$. 
\subsection{Convergence of Mutual Information for BIMS Channels}
To build intuition, we present a simple proof for the case when the DMC $W$ is a BIMS channel, with $P_X = \text{Ber}(1/2)$. The choice of the input distribution being uniform assumes relevance since the capacity of a BIMS channel is achieved by uniform inputs (see \cite[Problem 4.8]{mct}). 
%Hence, for this section, we concentrate on the rate $\rho(C)$, defined as $\rho(C):=\liminf_d -\frac{1}{d}\cdot \log \left(1 - C^{(d)}\right)$. 

The following bounds on the conditional entropy of the input to a BIMS channel given the output, which are drawn from \cite[Prop. 2.8]{sasoglufnt}, will prove useful. Recall the definition of the Bhattacharya parameter of a BIMS channel $W$ with output alphabet $\mathcal{Y}$ given by $Z_b(W) := \sum_{y\in \mathcal{Y}} \sqrt{P_{Y|0}(y)P_{Y|1}(y)}$.
\begin{lemma}
		\label{lem:sasoglu}
	Given a BIMS channel $\overline{W}$ with input $\overline{X}\sim P_X$, where $P_X =\text{Ber}(1/2)$, and output $\overline{Y}$, we have that 
	\[
		Z_b(\overline{W})^2\leq \mathsf{H}(\overline{X}\mid \overline{Y})\leq \log (1 + Z_b
		(\overline{W})).
	\]
\end{lemma}
We thus obtain the following simple corollary.
\begin{corollary}
	\label{cor:sasoglu}
	Given a BIMS channel $W$ with input $X\sim P_X$, where $P_X = \text{Ber}(1/2)$,  we have that for the $d$-view DMC $W^{(d)}$,
	\[
	Z_b({W})^{2d}\leq \mathsf{H}({X}\mid {Y^d})\leq Z_b({W})^d.
	\]
\end{corollary}
\begin{proof}
	We first note that when $W$ is a BIMS channel, then so is the $d$-view DMC $W^{(d)}$. Now, the Bhattacharya parameter
	\begin{align*}
		Z_b(W^{(d)})&= \sum_{y^d\in \mathcal{Y}^d} \sqrt{P_{Y|0}(y^d|0)P_{Y|1}(y^d|1)}\\
		&= \sum_{y^d\in \mathcal{Y}^d} \prod_{i=1}^d \sqrt{P_{Y|0}(y_i|0)P_{Y|1}(y_i|1)}\\
		&= \prod_{i=1}^d \sum_{y_i\in \mathcal{Y}} \sqrt{P_{Y|0}(y_i|0)P_{Y|1}(y_i|1)}\\
		&= Z_b(W)^d.
	\end{align*}
The proof is then completed by appealing to Lemma \ref{lem:sasoglu} and noting that $\log (1+z)\leq z$, for all $z> -1$.
\end{proof}

Moreover, we have the following bound on $\rho(I)$ for general binary-input DMCs and for arbitrary input distributions $P_X$.
\begin{lemma}
	\label{lem:bimsub}
	Given a binary-input DMC $W$ with input $X\sim P_X$, where $P_X$ is arbitrary, we have that
	\[
	\mathsf{H}(X|Y^d)\geq e^{-d\cdot \mathsf{C}(P_{Y\mid X=0},P_{Y\mid X=1})+\Theta(\log d)}.
	\]
\end{lemma}
\begin{proof}
	Observe that
	\begin{align*}
		\mathsf{H}(X|Y^d)&= \E\left[\log\frac{1}{P_{X\mid Y^{d}}(X\mid Y^{d})}\right].
		%& =P_{X}(0)\cdot\E\left[\log\frac{1}{P_{X\mid Y^{d}}(X=0\mid Y^{d})}\Bigg \vert X=0\right].
		%&\ \ \ \ \ \ \ \ \  +P_{X}(1)\cdot\E\left[\log\frac{1}{P_{X\mid Y^{d}}(X=1\mid Y^{d})}\Bigg \vert X=1\right].
	\end{align*}
%	Since $W$ is a BIMS channel, we have that
%	\[
%	\mathsf{H}(X|Y^d)=\E\left[\log\frac{1}{P_{X\mid Y^{d}}(X=0\mid Y^{d})}\Bigg \vert X=0\right].
%	\]
	Further, recall that in a binary Bayesian hypothesis testing setting (see \cite[Ch. 11]{cover_thomas}) with prior $P_{X}$
	and hypotheses $\{P_{Y\mid 0},P_{Y\mid 1}\}$, we have that the probability of correct decision is given by
	\[
	\E\left[P(X\mid Y^{d})\right]=1-e^{-d\cdot \mathsf{C}(P_{Y\mid X=0},P_{Y\mid X=1})+\Theta(\log d)}.
	\]
	Hence, we see that for large enough $d$,
	\begin{align}
		\mathsf{H}(X|Y^d) &= \E\left[\log\frac{1}{P(X\mid Y^{d})}\right] \notag\\ 
		& \geq-\log\left(1-e^{-d\cdot \mathsf{C}(P_{Y\mid X=0},P_{Y\mid X=1})+\Theta(\log d)}\right) \label{eq:inter}\\
		& \geq e^{-d\cdot \mathsf{C}(P_{Y\mid X=0},P_{Y\mid X=1})+\Theta(\log d)} \notag,
	\end{align}
	where the first inequality follows from Jensen's inequality and the second from the fact that $\log(1+z)\leq z$, for $z>-1$. Also, the $\Theta(\log d)$ term in the exponent in \eqref{eq:inter} is due either to the Laplace method (see \cite[Sec. 4.2]{nerifnt}) or to the results of \cite[Thm. 2.1 and Corollary 1]{arxivstat}. 
	
	%Hence, for any binary-input DMC, $\rho(I)\leq \mathsf{C}(P_{Y\mid X=0},P_{Y\mid X=1})$. 
\end{proof}
%\begin{remark}
%	One can obtain via  that the $o(d)$ term in \eqref{eq:inter} is in fact $\Theta(\log d)$.
%\end{remark}
The above ingredients suffice to afford a proof of Theorem \ref{thm:conv} for the special case of BIMS channels with a uniform input distribution.
\begin{proof}[Proof of Thm. \ref{thm:conv} for BIMS channels with uniform inputs]
	For the case when $W$ is a BIMS channel, we have that $\mathsf{C}(P_{Y|0},P_{Y|1}) = -\log Z_b(W)$ (see the remark following the statement of Theorem \ref{thm:conv}). Hence, when the input distribution is uniform, we have from Corollary \ref{cor:sasoglu}, we have that $\mathsf{H}(X|Y^d)\leq e^{-d\cdot \mathsf{C}(P_{Y|0},P_{Y|1})}$. The proof concludes by appealing then to Lemma \ref{lem:bimsub}, which shows that $\mathsf{H}(X|Y^d)\geq e^{-d\cdot \mathsf{C}(P_{Y|0},P_{Y|1})+\Theta(\log d)}$. Hence, overall, we have that $\mathsf{H}(X|Y^d)= e^{-d\cdot \mathsf{C}(P_{Y|0},P_{Y|1})+\Theta(\log d)}$.
\end{proof}
%\begin{remark}
%	By the Remark following the proof of Lemma \ref{lem:bimsub}, we see that for a BIMS channel $W$, $C^{(d)} = e^{-d\cdot Z_b(W)+\Theta(\log d)}$, thereby giving us a handle on higher-order asymptotics of the capacity.
%\end{remark}

It is possible, with some work, to present a proof of Theorem \ref{thm:conv} for $I^{(d)}$ for general DMCs with arbitrary input distributions with the aid of \cite[Lemma 9]{levenshtein} (see also \cite[Thm. 5]{shgalber}) and an extension of Lemma \ref{lem:bimsub}. However, the analysis of dispersion requires more involved techniques: we hence first present a proof for $I^{(d)}$ that introduces these techniques, in Section \ref{sec:gendmccap}, and then extend them to $V^{(d)}$, in Section \ref{sec:dispersion}.

\subsection{Convergence of Mutual Information for General DMCs}
\label{sec:gendmccap}
Given a general DMC $W$ with input alphabet $\mathcal{X}$ (not necessarily binary) and output alphabet $\mathcal{Y}$, consider the  $d$-view DMC $W^{(d)}$. Let the input to $W^{(d)}$ be $X$, with input distribution being $P_X$, and let its outputs be $Y_1,\ldots,Y_d \in \mathcal{Y}^d$. The joint distribution of the inputs and outputs is such that $P_{X,Y^d}(x,y^d) = P_X(x)\prod_{i=1}^d W(y_i|x)$. Much like the proof of Corollary \ref{cor:sasoglu}, the inequality
\[
\mathsf{H}(X|Y^d) \leq Z_g(W)^d,
\]
can be shown to hold (see \cite[Prop. 4.8]{sasoglufnt}), where $Z_g(W) := \sum_{x\neq x'} \sum_{y\in \mathcal{Y}} \sqrt{P(x)W(y|x)P(x')W(y|x')}$ is a scaled version of the Bhattacharya parameter for general DMCs. This then results in $\rho(I)\geq -\log Z_g(W)$, thereby showing that for well-behaved DMCs, the rate of convergence of $I^{(d)}$ to $H(X)$ is exponential in $d$. We shall now take up the question of the exact speed of this convergence.
	
To this end, we will be next interested in evaluating, up to exponential tightness, the behaviour of
\begin{align}
	\mathsf{H}(X|Y^d)&= \E\left[\log\frac{1}{P_{X\mid Y^{d}}(X\mid Y^{d})}\right] \notag\\
	& =\sum_{x\in \mathcal{X}}P_{X}(x)\E\left[\log\frac{1}{P_{X\mid Y^{d}}(x\mid Y^{d})}\Bigg \lvert X=x\right]. \label{eq:inter2}
\end{align}
Now, fix an $x\in \mathcal{X}$ and focus on the inner term in \eqref{eq:inter2}. Then,
\begin{align}
&\E\left[\log\frac{1}{P_{X\mid Y^{d}}(x\mid Y^{d})}\Bigg \lvert X=x\right] \notag\\ &\ \ \ \ \ \  \ \ \ \  \ \ =\int_{0}^{\infty}\P\left[\log\frac{1}{P_{X\mid Y^{d}}(x\mid Y^{d})}\geq t\Bigg \lvert X=x\right]\d t. \label{eq:inter3}
\end{align}
The inner probability, to wit, $p_x(t):=\P\left[-\log P_{X\mid Y^{d}}(x\mid Y^{d})\geq t \lvert X=x\right]$ is bounded as follows:
\begin{lemma}
	\label{lem:inter}
	We have that
	\begin{align*}
		&\frac{p_x(t)}{(|{\cal X}|-1)}\leq\max_{\tilde{x}\neq x}\P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq \frac{e^{-(t-\log(|{\cal X}|-1))}}{1-e^{-t}}\Bigg \lvert X=x\right],\\
		&\text{and}\\
		&p_x(t)	\geq \max_{\tilde{x}\neq x}\P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Bigg \lvert X=x\right].
	\end{align*}
\end{lemma}
\begin{proof}
	First, observe that
\begin{align*}
	& p_x(t)\\
	& =\P\left[\frac{P_{XY^{d}}(x,Y^{d})}{P_{Y^{d}}(Y^{d})}\leq e^{-t}\Bigg \lvert X=x\right]\\
	& =\P\left[P(x)P(Y^{d}\mid x)\leq e^{-t}\sum_{\tilde{x}}P(\tilde{x})P(Y^{d}\mid\tilde{x})\Big \lvert X=x\right]\\
	& =\P\left[\frac{P(x)P(Y^{d}\mid x)}{\sum_{\tilde{x}\neq x}P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Big \lvert X=x\right].
\end{align*}
We first prove the upper bound in the lemma. The above probability obeys
\begin{align*}
	& \P\left[\frac{P(x)P(Y^{d}\mid x)}{\sum_{\tilde{x}\neq x}P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Bigg \lvert X=x\right]\\
	& \leq\P\left[\frac{P(x)P(Y^{d}\mid x)}{(|{\cal X}|-1)\max_{\tilde{x}\neq x}P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Bigg \lvert X=x\right]\\
	& =\P\left[\frac{1}{|{\cal X}|-1}\cdot\min_{\tilde{x}\neq x}\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Bigg \lvert X=x\right]\\
	& \leq\sum_{\tilde{x}\neq x}\P\left[\frac{1}{|{\cal X}|-1}\cdot\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Bigg\lvert X=x\right]\\
	& \leq(|{\cal X}|-1)\cdot\max_{\tilde{x}\neq x}\P\left[\frac{1}{|{\cal X}|-1}\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\Bigg \lvert X=x\right],
\end{align*}
thereby showing the upper bound. Further, for any $\tilde{x}$, we have that
\begin{align*}
p_x(t) &=
\P\left[\frac{P(x)P(Y^{d}\mid x)}{\sum_{\tilde{x}\neq x}P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\mid X=x\right]\\
&\geq\max_{\tilde{x}\neq x}\P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-t}}{1-e^{-t}}\mid X=x\right],
\end{align*}
thereby proving the lower bound.
\end{proof}
Since we are interested mainly in the behaviour of $\mathsf{H}(X|Y^d)$ upto first order in the exponent $d$, it suffices for us to understand the behaviour of $p_x(t)$ upto first order in the exponent $d$ with the expectation that we will accrue an additional $\Theta(\log d)$ term in the exponent, in the final expression (see Eq. \eqref{eq:inter3} above and  \cite[Sec. 4.2]{nerifnt} for intuition). To this end, following Lemma \ref{lem:inter}, for fixed $z\in [0,\infty)$ and $c>0$, we shall focus on the term
\[
\Gamma_{x,\tilde{x}}(z):= \P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq \frac{ce^{-z}}{1-e^{-z}}\Bigg \lvert X=x\right],
\]
with the reasoning that the rate of convergence of $\mathsf{H}(X|Y^d)$ will be dictated by the smallest rate of $\Gamma_{x,\tilde{x}}(z)$, as $z$ increases from $0$ to $\infty$.
%The upper and lower bound match up to constants $|{\cal X}|$ (which
%slightly affect the probability, or the value of $t$ (because it
%changes $e^{-t}$ to $e^{-t+\log(|{\cal X}|-1)}$ and $t$ will be
%linear with $d$). 
%Thus, we next analyze the probability in the lower
%bound. 

Before we proceed, we require some more notation. Let us denote the log-likelihood ratio by 
\[
L_{x,\tilde{x}}^y:=\log\frac{P_{Y\mid X}(y\mid x)}{P_{Y\mid X}(y\mid\tilde{x})}.
\]
For a given $y^{d}\in{\cal Y}^{d}$ and for $b\in \mathcal{Y}$, let
$\hat{Q}_{y^{d}}(b):=\frac{1}{d}\sum_{i=1}^{d}\mathds{1}\{y_{i}=b\}$ be the empirical frequency of the letter $b$ in any output sequence. Further, we define
\[
L_{x,\tilde{x}}(\hat{Q}):=\sum_{b\in{\cal Y}}\hat{Q}(b)L_{x,\tilde{x}}^b.
\]
Finally, let 
\[
v_{x,\tilde{x}}\equiv v_{x,\tilde{x}}(z) := \frac{1}{d}\left(\log\left(\frac{ce^{-z}}{1-e^{-z}}\right) - \log \frac{P(x)}{P(\tilde{x})}\right)
\]
and let $z(v_{x,\tilde{x}}):= \log\left(1+\frac{cP(\tilde{x})}{P(x)}\cdot e^{-dv_{x,\tilde{x}}}\right)$ be its inverse function.
%Since the upper and lower bound are rather similar, we set a pair
%$x,\tilde{x}$ and turn to analyze
\begin{proposition}
	\label{prop:Gamma}
	We have that for any fixed $\delta>0$,
	\begin{enumerate}
		\item If $v_{x,\tilde{x}}\geq L_{x,\tilde{x}}({P_{Y|x}}) + \delta$, then $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) = \Theta(1)$.
		\item If $v_{x,\tilde{x}}\leq L_{x,\tilde{x}}({P_{Y|x}})-\delta$, then $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) = e^{-dE(v_{x,\tilde{x}})+\Theta(\log d)}$, where
		\[
		E(v_{x,\tilde{x}}):=
		\begin{cases}
			\max_{\lambda\geq 0}\left[-\log \left(\sum_{y} P(y|x)^{1-\lambda}P(y|x')^\lambda\right)-\lambda v_{x,\tilde{x}}\right],\\ \ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \  \ \ \ \ \ \ \ \  \text{if }v_{x,\tilde{x}}\geq \min_{b\in \mathcal{Y}} L_{x,\tilde{x}}^b,\\
			\infty,\ \text{otherwise}.
		\end{cases}
		\]
	\end{enumerate}
\end{proposition}
\begin{proof}
Observe that for any $z\in [0,\infty)$,
\begin{align*}
	&\Gamma_{x,\tilde{x}}(z)\\&= \P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq \frac{ce^{-z}}{1-e^{-z}}\Bigg \lvert X=x\right]\\
	& =\P\left[\sum_{i=1}^{d}\log\frac{P_{Y\mid X}(Y_{i}\mid x)}{P_{Y\mid X}(Y_{i}\mid\tilde{x})}\leq\log\left(\frac{ce^{-z}}{1-e^{-z}}\right) - \log \frac{P(x)}{P(\tilde{x})}\Bigg \lvert X=x\right]\\
	& =\P\left[\sum_{i=1}^{d}L_{x,\tilde{x}}^{Y_{i}}\leq\log\left(\frac{ce^{-z}}{1-e^{-z}}\right)- \log \frac{P(x)}{P(\tilde{x})}\Bigg \lvert X=x\right]\\
	& =\P\left[\E_{\hat{Q}}\left[L_{x,\tilde{x}}^{Y^{d}}\right]\leq v_{x,\tilde{x}}(z)\Big \lvert X=x\right].
\end{align*}
Writing this differently, we have that for any $v_{x,\tilde{x}}\in \mathbb{R}$,
\[
\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) = \P\left[\E_{\hat{Q}}\left[L_{x,\tilde{x}}^{Y^{d}}\right]\leq v_{x,\tilde{x}}\Big \lvert X=x\right].
\]
Consider first the case when $v_{x,\tilde{x}}\geq L_{x,\tilde{x}}({P_{Y|x}}) + \delta$. Note that $L_{x,\tilde{x}}({P_{Y|x}}) = D(P_{Y|x}||P_{Y|\tilde{x}})>0$. We split this case into two subcases.
\begin{itemize}
	\item If $v_{x,\tilde{x}}\geq\max_{b\in{\cal Y}}L_{x,\tilde{x}}^b$ then $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) = 1$. 
	\item Otherwise, consider the case where $L_{x,\tilde{x}}(P_{Y\mid x})+\delta\leq v_{x,\tilde{x}}\leq\max_{b\in{\cal Y}}L_{x,\tilde{x}}^b$. Now, observe that
	\begin{align*}
	1\geq \Gamma_{x,\tilde{x}}(&z(v_{x,\tilde{x}}))\geq\\ &\P \left[\E_{\hat{Q}}\left[L_{x,\tilde{x}}^{Y^{d}}\right]\leq L_{x,\tilde{x}}(P_{Y\mid x})+\delta\Big \lvert X=x\right].
	\end{align*}
	Furthermore, by a simple application of Markov's inequality, we get that since $L_{x,\tilde{x}}(P_{Y\mid x}) = \E_{Y^d\sim P_{Y^d|x}}[L_{x,\tilde{x}}^{Y^d}]$, the following inequality holds:
	\[
	\P \left[\E_{\hat{Q}}\left[L_{x,\tilde{x}}^{Y^{d}}\right]\leq L_{x,\tilde{x}}(P_{Y\mid x})+\delta\Big \lvert X=x\right]\geq \frac{\delta}{L_{x,\tilde{x}}(P_{Y\mid x})+\delta}.
	\]
	Hence, we have that $1\geq \Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) \geq \frac{\delta}{L_{x,\tilde{x}}(P_{Y\mid x})+\delta}$.
\end{itemize}
Hence, overall, if $v_{x,\tilde{x}}\geq L_{x,\tilde{x}}({P_{Y|x}}) + \delta$, we get that $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) = \Theta(1)$.

Next, consider the case when $v_{x,\tilde{x}}\leq L_{x,\tilde{x}}({P_{Y|x}}) - \delta$. We again split this case into two subcases.
\begin{itemize}
	\item If $v_{x,\tilde{x}}\leq\min_{b\in{\cal Y}}L_{x,\tilde{x}}^b$, then $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) = 0$.
	\item If $\min_{b\in{\cal Y}}L_{x,\tilde{x}}^b\leq v_{x,\tilde{x}}\leq L_{x,\tilde{x}}(P_{Y\mid X=x})$,
	then this is a large-deviations event. The probability $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}}))$ thus decays
	exponentially in $d$, i.e., $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}})) \doteq e^{-dE_1(v_{x,\tilde{x}})+\Theta(\log d)}$, for some $E_1:\mathbb{R}\to [0,\infty)$, where by Sanov's theorem (see \cite[Sec. 11.4]{cover_thomas}), we have that $E_1(v_{x,\tilde{x}}) = \min_{Q\colon L_{x,\tilde{x}}(Q)\leq v_{x,\tilde{x}}}D(Q\mid\mid P_{Y\mid X=x})$. We now aim to characterize this function $E_1$.
	
	From convex duality (see \cite[Sec. 5.2]{boyd}), we obtain that 
	\begin{equation}
		\label{eq:E1}
	E_1(v_{x,\tilde{x}}) = \max_{\lambda\geq0}\min_{Q}D(Q\mid\mid P_{Y\mid X=x})+\lambda(L_{x,\tilde{x}}(Q)-v_{x,\tilde{x}}).
	\end{equation}
	First, let us solve the inner minimization. Fix $\lambda\geq 0$. Observe that the term $f(\lambda,Q):= D(Q\mid\mid P_{Y\mid X=x}) + \lambda L_{x,\tilde{x}}(Q)$ obeys
	\begin{align*}
		f(\lambda,Q)&=\sum_{y}Q(y)\left(\log\frac{Q(y)}{P_{Y\mid X=x}(y)}+\lambda L_{x,\tilde{x}}(y)\right)\\
		 & =-\sum_{y}Q(y)\left(\log\frac{P_{Y\mid X=x}(y)}{Q(y)e^{\lambda L_{x,\tilde{x}}(y)}}\right)\\ &\geq-\log\sum_{y}\frac{P_{Y\mid X=x}(y)}{e^{\lambda L_{x,\tilde{x}}(y)}},
	\end{align*}
	using Jensen's inequality. Also note that equality holds when $Q(y) = Q^*(y)=\frac{1}{Z_{x,\tilde{x}}(\lambda)}P_{Y\mid X=x}(y)e^{-\lambda L_{x,\tilde{x}}(y)}$, where $Z_{x,\tilde{x}}(\lambda) := \sum_{y\in \mathcal{Y}} P_{Y\mid X=x}(y)e^{-\lambda L_{x,\tilde{x}}(y)}$ is the partition function (normalization constant). Substituting $Q^*$ back into the function results 
	\begin{align*}
		f(\lambda,Q^*)&=-\log Z_{x,\tilde{x}}(\lambda) -\lambda v_{x,\tilde{x}}\\
		& =-\log\left(\sum_{y}P_{Y\mid X=x}(y)e^{-\lambda L_{x,\tilde{x}}(y)}\right)-\lambda v_{x,\tilde{x}}\\
		& =-\log\left(\sum_{y}P_{Y\mid X=x}^{1-\lambda}(y\mid x)P_{Y\mid X}^{\lambda}(y\mid\tilde{x})\right)-\lambda v_{x,\tilde{x}}.
	\end{align*}
	Plugging back into \eqref{eq:E1}, we get that 
	\begin{align*}
	&E_1(v_{x,\tilde{x}})\\ &= \max_{\lambda\geq0} \Bigg[-\log\left(\sum_{y}P_{Y\mid X=x}^{1-\lambda}(y\mid x)P_{Y\mid X}^{\lambda}(y\mid\tilde{x})\right) -\lambda v_{x,\tilde{x}}\Bigg].
	\end{align*}
\end{itemize}
Note that by setting $E(v_{x,\tilde{x}}) = E_1(v_{x,\tilde{x}})$ when $\min_{b\in{\cal Y}}L_{x,\tilde{x}}^b\leq v_{x,\tilde{x}}\leq L_{x,\tilde{x}}(P_{Y\mid X=x})$ and $E(v_{x,\tilde{x}}) = \infty$ when $v_{x,\tilde{x}}\leq\min_{b\in{\cal Y}}L_{x,\tilde{x}}^b$, we obtain a tight characterization of the rate of exponential decay of $\Gamma_{x,\tilde{x}}(z(v_{x,\tilde{x}}))$, in these ranges of $v_{x,\tilde{x}}$.
\end{proof}
%The two first cases can be combined because in both cases the probability
%is $\Theta(1)$, and also the third and four cases, by allowing the
%exponent to be infinite in case $\{Q:L(Q)\leq v_{x,\tilde{x}}\}$ is an empty set. 
We now state a prove a lemma that will allow us to identify the exact rate of exponential decay of $\mathsf{H}(X|Y^d)$.
\begin{lemma}
	\label{lem:inter2}
	We have that
	\[
	\int_{0}^{\infty} \max_{\tilde{x}\neq x} \Gamma_{x,\tilde{x}}(z) \d z = e^{\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\cdot e^{-d\cdot \min_{\tilde{x}\neq x} \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})}.
	\]
\end{lemma}
\begin{proof}
	Consider an integral of the form
	\[
	\overline{I} = \int_{0}^{\infty} \max_{\tilde{x}\neq x} \Gamma_{x,\tilde{x}}(z) \d z.
	\]
	First, observe that 
	\begin{align*}
	\overline{I} &\leq \int_{0}^{\infty} \sum_{\tilde{x}\neq x}\Gamma_{x,\tilde{x}}(z) \d z\\
	 &\leq |\mathcal{X}|^2\cdot \max_{\tilde{x}\neq x}\int_{0}^{\infty} \Gamma_{x,\tilde{x}}(z) \d z\\
	 &=e^{\Theta(\log |\mathcal{X}|)}\cdot \max_{\tilde{x}\neq x}\int_{0}^{\infty} \Gamma_{x,\tilde{x}}(z) \d z.
	\end{align*}
Further,
\begin{align*}
	\overline{I} &\geq \max_{\tilde{x}\neq x}\int_{0}^{\infty} \Gamma_{x,\tilde{x}}(z) \d z.
\end{align*}
Hence, overall, we have that $\overline{I} = \text{exp}(\Theta(\log|\mathcal{X}|))\cdot \max_{\tilde{x}\neq x}\int_{0}^{\infty} \Gamma_{x,\tilde{x}}(z) \d z$. We next focus on the integral
\[
I = \int_{0}^{\infty} \Gamma_{x,\tilde{x}}(z) \d z,
\]
for a fixed $x, \tilde{x}$. 

By the definition $v_{x,\tilde{x}} = v_{x,\tilde{x}}(z) = \frac{1}{d}\left(\log\left(\frac{ce^{-z}}{1-e^{-z}}\right) - \log \frac{P(x)}{P(x')}\right)$ and from Prop. \ref{prop:Gamma}, we see that the integral $I$ can be split into two integrals for its evaluation: integral $I_1$, when $z\leq \log \left(1+\frac{cP(\tilde{x})}{P(x)}\cdot e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)}\right):=u(d)$ (or equivalently, $v_{x,\tilde{x}}\geq  L_{x,\tilde{x}}({P_{Y|x}}) + \delta$), and integral $I_2$, when $z\geq \log \left(1+\frac{cP(\tilde{x})}{P(x)}\cdot e^{-d(L_{x,\tilde{x}}(P_{Y|x})-\delta)}\right):=\ell(d)$ (or equivalently, $v_{x,\tilde{x}}\leq  L_{x,\tilde{x}}({P_{Y|x}}) - \delta$), with $I = I_1+I_2$. Here, we pick $\delta< L_{x,\tilde{x}}({P_{Y|x}})$.

Consider first the integral $I_1$. We have that
	\begin{align*}
		I_1 &= \int_{z\leq u(d)}  \Gamma_{x,\tilde{x}}(z) \d z\\
		&= \Theta(1)\cdot  u(d).
	\end{align*}
Now, we claim that $u(d)= e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)+\Theta(\log d)}$. To see this, let $\tilde{c}:= \frac{cP(\tilde{x})}{P(x)}$ and observe that from standard identities involving the $\log$ function,
\[
u(d)\leq \tilde{c}e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)},
\]
and
\[
u(d)\geq  \frac{\tilde{c}e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)}}{1+\tilde{c}e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)}} \geq \frac{\tilde{c}}{2}\cdot e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)},
\]
since $L_{x,\tilde{x}}({P_{Y|x}}) = D(P_{Y|x}||P_{Y|\tilde{x}})>0$. 
Hence, overall, we have that for any fixed $\delta>0$, $I_1 =  e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)+\Theta(1)}$. Taking the limit as $\delta \downarrow 0$, we get that 
\begin{equation}I_1=  e^{-dL_{x,\tilde{x}}(P_{Y|x})+\Theta(1)} =  e^{-d\cdot D(P_{Y|x}||P_{Y|\tilde{x}})+\Theta(1)}.  \label{eq:i1} \end{equation}

Consider now the integral $I_2$. Note that from case 2) in Prop. \ref{prop:Gamma}, when $z\geq  \log \left(1+\tilde{c}e^{-d\cdot \min_b L_{x,\tilde{x}}^b}\right):=U(d)$, we have that $I_2 = 0$. Hence, we can write
\[
I_2 = \int_{\ell(d)\leq z\leq U(d)}  \Gamma_{x,\tilde{x}}(z) \d z,
\]
where, for this interval $\ell(d)\leq z\leq U(d)$ of interest, 
\[
\Gamma_{x,\tilde{x}}(z) = e^{-d{E}(v_{x,\tilde{x}}(z))+\Theta(\log d)},
\]
with \begin{equation}{E}(v_{x,\tilde{x}}(z)) = \max_{\lambda\geq 0}\left[-\log \left(\sum_{y} P(y|x)^{1-\lambda}P(y|x')^\lambda\right)-\lambda v_{x,\tilde{x}}\right],\label{eq:E}\end{equation} from Prop. \ref{prop:Gamma}.

It is clear that $E(v_{x,\tilde{x}}(z))$ increases as $v_{x,\tilde{x}}$ decreases. In the integral $I_2$, we thus make the change of variables
\[
v = \frac{1}{d}\left(\log\left(\frac{ce^{-z}}{1-e^{-z}}\right) - \log \frac{P(x)}{P(x')}\right),
\]
with $\d z = \frac{-dc e^{-dv}}{1+ce^{-dv}} \d v$. Thus,
\begin{align*}
	I_2 &=  dc\int^{L_{x,\tilde{x}}(P_{Y|x})-\delta}_{v=\min_b L_{x,\tilde{x}}^b} e^{-dE(v)} \cdot \frac{e^{-dv}}{1+ce^{-dv}} \d v\\
	&= dc\int^{L_{x,\tilde{x}}(P_{Y|x})-\delta}_{v=0} e^{-dE(v)}\cdot   \frac{e^{-dv}}{1+ce^{-dv}} \d v + \\
	&\ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \  dc\int^{0}_{v=\min_b L_{x,\tilde{x}}^b} e^{-dE(v)}\cdot \frac{e^{-dv}}{1+ce^{-dv}} \d v.
\end{align*}
Let us call the first integral in the expansion above as $I_{2,a}$ and the second as $I_{2,b}$ (note that $\min_b L_{x,\tilde{x}}^b\leq 0$). Now, observe that 
\begin{align*}
	I_{2,a}&=dc\int^{L_{x,\tilde{x}}(P_{Y|x})-\delta}_{v=0} e^{-dE(v)}\cdot {e^{-dv+\Theta(\log d)}} dv\\
	&= \text{exp}(-d(E(L_{x,\tilde{x}}(P_{Y|x})) + L_{x,\tilde{x}}(P_{Y|x})-\delta)+\Theta(\log d)).
\end{align*}
Here, in the first eqauility, we argue as previously that 
\[
\frac{e^{-dv}}{1+ce^{-dv}} = e^{-dv+\Theta(1)}.
\]
Furthermore, the second equation follows from Laplace's method (e.g., see \cite[Sec. 4.2]{nerifnt}), using the fact that both $e^{-dE(v)}$ and $e^{-dv}$ increase as $v$ increases. Taking $\delta\downarrow 0$, we obtain that
\begin{equation}
	I_{2,a}= e^{-d(E(L_{x,\tilde{x}}(P_{Y|x})) + L_{x,\tilde{x}}(P_{Y|x}))+\Theta(\log d)}.
	\label{eq:i2a}
\end{equation}

Moreover,
\begin{align}
	I_{2,b} &=e^{\Theta(\log d)}\cdot \int^{0}_{v=\min_b L_{x,\tilde{x}}^b}e^{-dE(v)} \d v \notag\\
	&\doteq e^{-dE(0)+\Theta(\log d)} = e^{-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)}. \label{eq:i2b}
\end{align}
Here, for the first equality, we use the fact that when $v\leq 0$, 
\[
\frac12\leq \frac{e^{-dv}}{1+ce^{-dv}} \leq \frac{1}{c},
\]
and hence $\frac{e^{-dv}}{1+ce^{-dv}} = \Theta(1)$.
The second equality holds again by Laplace's method, using the fact that $e^{-dE(v)}$ increases with $v$.

Putting everything together, in order to nail down the exponential behaviour of integral $I$, we need to reconcile Equations \eqref{eq:i1}, \eqref{eq:i2a}, and \eqref{eq:i2b}, to understand which among $I_1$, $I_{2,a}$, and $I_{2,b}$, is the largest. First, observe that since $\mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})\leq D(P_{Y|x}||P_{Y|\tilde{x}})$, we have that $I_{2,b}$ dominates $I_1$.

Therefore, the exponential behaviour of integral $I$ is governed by the rate
\[
\overline{E} = \min \left\{E(L_{x,\tilde{x}}(P_{Y|x})) + L_{x,\tilde{x}}(P_{Y|x}), \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}}) \right\}.
\]
Now note that the maximum over $\lambda \geq 0$ in the expressions for $E$ and $\mathsf{C}$ can be rewritten as a maximum over $\lambda \in [0,1]$ (owing to the concavity of $-\log \left(\sum_{y} P(y|x)^{1-\lambda}P(y|x')^\lambda\right)$ and the fact that it equals $0$ at $\lambda = 0,1$). We then get that
\[
E(L_{x,\tilde{x}}(P_{Y|x})) + L_{x,\tilde{x}}(P_{Y|x})\geq \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}}),
\]
implying that $\overline{E} = \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})$. Therefore, $I= e^{-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)}$, and hence that $\overline{I}= \max_{\tilde{x}\neq x} \text{exp}({-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)})$. 
\end{proof}
We are now ready to prove Theorem \ref{thm:conv} for the convergence of the mutual information.
\begin{proof}[Proof of Thm. \ref{thm:conv} for mutual information]
Recall from Lemma \ref{lem:inter} that
\[
p_x(t)\leq (|\mathcal{X}|-1)\cdot\max_{\tilde{x}\neq x}\Gamma_{x,\tilde{x}}(t),
\]
with the constant $c$ in the definition of $\Gamma_{x,\tilde{x}}(t)$ taken to be $|\mathcal{X}|-1$. Thus, from Lemma \ref{lem:inter2} and \eqref{eq:inter3}, we get that
\begin{align*}
&\E\left[\log\frac{1}{P_{X\mid Y^{d}}(x\mid Y^{d})}\Bigg \lvert X=x\right]\\  &= \int_{0}^\infty p_x(t)\d t\\ &\leq \text{exp}\left({-d\cdot \min_{\tilde{x}\neq x} \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right),
\end{align*}
where the inequality holds by the Laplace method  \cite[Sec. 4.2]{nerifnt}.
Similarly, since
\[
p_x(t)\geq \max_{\tilde{x}\neq x} \Gamma_{x,\tilde{x}}(t),
\]
with the constant $c$ in the definition of $\Gamma_{x,\tilde{x}}(t)$ taken to be $1$, we get that
\begin{align*}
&\E\left[\log\frac{1}{P_{X\mid Y^{d}}(x\mid Y^{d})}\Bigg \lvert X=x\right]\\  &\geq \text{exp}\left({-d\cdot \min_{\tilde{x}\neq x} \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right).
\end{align*}
Thus,
\begin{align*}
&\E\left[\log\frac{1}{P_{X\mid Y^{d}}(x\mid Y^{d})}\Bigg \lvert X=x\right]\\&= \text{exp}\left({-d\cdot \min_{\tilde{x}\neq x} \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right).
\end{align*}
Plugging back in \eqref{eq:inter2}, we obtain that $\mathsf{H}(X|Y^d)= \max_{\substack{x,\tilde{x}: \tilde{x}\neq x}} \text{exp}\left({-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right)$, yielding the required result.
\end{proof}

\section{Convergence of Channel Dispersion}
\label{sec:dispersion}

We now shift our attention to proving the convergence of the dispersion $V^{(d)} = \mathbb{E}\left[\left(\iota(X;Y^d) - I(X;Y^d)\right)^2\right]$, to the varentropy $\mathsf{V}(X)$ of the input distribution $P_X$, for general DMCs $W$. 
	
First, we write
\begin{align}
		&V^{(d)} \notag\\ &= \E\left[\left(\log \frac{P(X|Y^d)}{P(X)} - \left(\mathsf{H}(X) - \mathsf{H}(X|Y^d)\right)\right)^2\right]\notag\\
		&= \E\left[\left(\log \frac{1}{P(X)} - H(X)\right)^2\right] + \E\left[\left(\log P(X|Y^d) + \mathsf{H}(X|Y^d)\right)^2\right]\notag\\
		&\ \ \ + 2\cdot\E\left[(\log P(X|Y^d)+\mathsf{H}(X|Y^d))\cdot \left(\log \frac{1}{P(X)} - H(X)\right)\right]\notag\\
		&= \mathsf{V}(X)+\left(\E\left[\left(\log P(X|Y^d)\right)^2\right] - \mathsf{H}(X|Y^d)^2\right)+\theta_d, \label{eq:interdisp}
\end{align}
where we use the fact that $\E\left[-\log P(X|Y^d)\right] = \mathsf{H}(X|Y^d)$, and the cross-term $\theta_d$ is
\[
2\cdot\E\left[(\log P(X|Y^d)+\mathsf{H}(X|Y^d))\cdot \left(\log \frac{1}{P(X)} - H(X)\right)\right].
\]

Further, observe that when $P_X = \text{Unif}(\mathcal{X})$, the cross term vanishes, since for any $x\in \mathcal{X}$, we have that $\log \frac{1}{P(x)} = \log |\mathcal{X}| = \mathsf{H}(X)$. Our proof strategy hence is to first characterize (upto exponential tightness) the behaviour of $\E\left[\left(\log P(X|Y^d)\right)^2\right]$ and then handle the cross-term $\theta_d$.
\begin{lemma}
	\label{lem:interdisp1}
	We have that
	\[
	\E\left[\left(\log P(X|Y^d)\right)^2\right]= e^{\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\cdot \max_{x,\tilde{x}: \tilde{x}\neq x} e^{-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})}.
	\]
\end{lemma}
\begin{proof}
	This proof is entirely analogous to the proof of convergence of $I^{(d)}$ to $\mathsf{H}(X)$, for general DMCs, in Section \ref{sec:gendmccap}, and we only highlight the key steps.
	
	We first consider the term $\E\left[\left(\log P(X|Y^d)\right)^2\right]$. As in \eqref{eq:inter2}, we first expand this term as:
	\[
	\E\left[\left(\log P(X|Y^d)\right)^2\right] = \sum_{x\in \mathcal{X}}P(x)\E\left[\left(\log P(X|Y^d)\right)^2\Bigg \lvert X=x\right],
	\]
	where for any $x\in \mathcal{X}$, we have
	\begin{align*}
	&\E\left[\left(\log P(x|Y^d)\right)^2\Bigg \lvert X=x\right]\\ &= \int_{t=0}^\infty \Pr\left[\left(\log P(x|Y^d)\right)^2 \geq t \Bigg \lvert X=x\right] \d t\\
	&= \int_{t=0}^\infty \P\left[\log P(x|Y^d)\geq \sqrt{t}\Big \lvert X=x\right] \d t +\\
	&\ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \  \  \int_{t=0}^\infty \P\left[\log P(x|Y^d)\leq -\sqrt{t}\Big \lvert X=x\right] \d t\\
	&= \int_{t=0}^\infty \P\left[\log P(x|Y^d)\leq -\sqrt{t}\Big \lvert X=x\right] \d t.
	\end{align*}
Here, the last equality holds since $P(x|Y^d)\leq 1$, for any $Y^d\in \mathcal{Y}^d$. As earlier, our task reduces to understanding the exponential behaviour of $q_x(t):= \Pr\left[\log P(x|Y^d)\leq -\sqrt{t}\Big \lvert X=x\right]$.

Exactly as in Lemma \ref{lem:inter}, we have that
\begin{align*}
	&\frac{q_x(t)}{(|{\cal X}|-1)}\\ &\leq\max_{\tilde{x}\neq x}\P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq \frac{e^{-(\sqrt{t}-\log(|{\cal X}|-1))}}{1-e^{-\sqrt{t}}}\Bigg \lvert X=x\right],\\
	\text{and}\\
	&q_x(t)	\geq \max_{\tilde{x}\neq x}\P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq\frac{e^{-\sqrt{t}}}{1-e^{-\sqrt{t}}}\Bigg \lvert X=x\right].
\end{align*}
Consider, for a fixed $c>0$ and $z\in [0,\infty)$, the expression
\[
\Delta_{x,\tilde{x}}(z):= \P\left[\frac{P(x)P(Y^{d}\mid x)}{P(\tilde{x})P(Y^{d}\mid\tilde{x})}\leq \frac{ce^{-\sqrt{z}}}{1-e^{-\sqrt{z}}}\Bigg \lvert X=x\right].
\]
As argued in the case of the mutual information, the rate of exponential decay of $\Delta_{x,\tilde{x}}(z)$, as a function of $z$, dictates the rate of exponential decay of $q_x(t)$, and hence of $\E\left[\left(\log P(X|Y^d)\right)^2\right]$. Once again, letting $v_{x,\tilde{x}} = v_{x,\tilde{x}}(z) = \frac{1}{d}\left(\log\left(\frac{ce^{-z}}{1-e^{-z}}\right) - \log \frac{P(x)}{P(x')}\right)$ and setting $(z(v_{x,\tilde{x}}))^{1/2}:= \log\left(1+\frac{cP(\tilde{x})}{P(x)\cdot }e^{-dv_{x,\tilde{x}}}\right)$, we obtain a result similar to Proposition \ref{prop:Gamma}, with the only modification being the replacement of $\Gamma_{x,\tilde{x}}$ by $\Delta_{x,\tilde{x}}$.

Next, as in Lemma \ref{lem:inter2}, consider the integral
\[
\overline{I}^{V} = \int_{0}^{\infty} \max_{\tilde{x}\neq x} \Delta_{x,\tilde{x}}(z) \d z.
\]
We claim that $\overline{I}^{V} = e^{\Theta(\log d)+\Theta(\log |\mathcal{X})}\cdot e^{-d \min_{\tilde{x}\neq x} \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})}$. To obtain this, we argue as in the proof of Lemma \ref{lem:inter2} that $\overline{I}^{V} = e^{\Theta(\log |\mathcal{X}|)}\cdot \max_{\tilde{x}\neq x} I^V$, where
\[
I^V = \int_{0}^{\infty} \Delta_{x,\tilde{x}}(z) \d z,
\]
for a fixed $x, \tilde{x}$.

Now, we split the evaluation of $I^V$ into two integrals: integral $I_1^V$, when $z\leq \left(\log \left(1+\frac{cP(\tilde{x})}{P(x)}\cdot e^{-d(L_{x,\tilde{x}}(P_{Y|x})+\delta)}\right)\right)^2$, and integral $I_2^V$, when $z\geq \left(\log \left(1+\frac{cP(\tilde{x})}{P(x)}\cdot e^{-d(L_{x,\tilde{x}}(P_{Y|x})-\delta)}\right)\right)^2$, with $I^V = I_1^V+I_2^V$. By arguments analogous to those in the proof of Lemma \ref{lem:inter2}, we obtain that 
\[
I_1^V= e^{-2d\cdot D(P_{Y|x}||P_{Y|\tilde{x}})+\Theta(\log d)},
\]
and
\[
I_2^V= e^{-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)}.
\]
Thus, we have that $I^V = e^{-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)}$, and hence that $\overline{I}^V = \text{exp}\left({-d\cdot \min_{\tilde{x}\neq x} \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right)$. Putting everything togehter, we get that $\E\left[\left(\log P(X|Y^d)\right)^2\right]= \max_{x,\tilde{x}: \tilde{x}\neq x} \text{exp}\left({-d\cdot  \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right)$.
\end{proof}

\begin{lemma}
	\label{lem:interdisp2}
	We have that
	\[
	\theta_d=  \max_{x,\tilde{x}: \tilde{x}\neq x}  e^{-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)}.
	\]
\end{lemma}
\begin{proof}
Recall that the cross term $$\theta_d:= 2\cdot \E\left[(\log P(X|Y^d)+\mathsf{H}(X|Y^d))\cdot \left(\log \frac{1}{P(X)} - H(X)\right)\right].$$ 

We then write
\begin{align*}
&\theta_d(x)\\ &:= \left(\log \frac{1}{P(x)} - H(X)\right)\cdot \left(\E\left[\log P(x|Y^d)\Big \lvert X=x\right]+\mathsf{H}(X|Y^d)\right),
\end{align*}
with $\theta_d = \sum_{x\in \mathcal{X}}P(x)\theta_d(x)$. From the capacity analysis, we know that (see \eqref{eq:inter3}) 
\begin{align*}&\E\left[\log P(x|Y^d)\Big \lvert X=x\right]\\ &= -\max_{x'\neq x}\text{exp}\left({-d\cdot  \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right).\end{align*} From our previous analysis, we know that $\mathsf{H}(X|Y^d)= \max_{x,x': x'\neq x} \text{exp}\left({-d\cdot  \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right)$. Hence,
 \begin{align*}\theta_d&= e^{\Theta(\log d)}\cdot\theta_d(x)\\ &= \max_{x,x': x\neq x'}\text{exp}\left({-d\cdot  \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right).\end{align*}
\end{proof}
With these lemmas in place, the proof of Theorem is easily completed.
\begin{proof}[Proof of Thm. \ref{thm:conv} for dispersion]
	From \eqref{eq:interdisp} we see that
	\[
	V^{(d)}-\mathsf{V}(X)= \E\left[\left(\log P(X|Y^d)\right)^2\right] - \mathsf{H}(X|Y^d)^2+\theta_d.
	\]
	Putting together Lemmas \ref{lem:interdisp1} and \ref{lem:interdisp2} and the fact that $\mathsf{H}(X|Y^d)= \max_{\substack{x,x': x'\neq x}} \text{exp}\left({-d\cdot \mathsf{C}(P_{Y|x},P_{Y|\tilde{x}})+\Theta(\log d)+\Theta(\log |\mathcal{X}|)}\right)$ (from the proof of Thm. \ref{thm:conv} for mutual information), we readily obtain the required result.
\end{proof}

==> main-results.tex <==
\label{sec:main}


==> poisson.tex <==
\label{sec:poisson}
In this section, we take up the special case of the $d$-view BSC$(p)$, denoted by $\text{BSC}^{(d)}(p)$. Recall that the capacity of this channel equals the capacity of the binomial channel $\mathsf{Bin}_d(p)$, which is given in \eqref{eq:bin}. Our objective is to show that the Poisson approximation channel $\mathsf{Poi}_d(p)$ introduced in Section  \ref{sec:main} has capacity that is a very good lower bound on the capacity of $\text{BSC}^{(d)}(p)$, via the proof of Theorem \ref{thm:poibin}. Before we proceed with the proof, we state and prove a simple lemma about the concavity of the mutual information $I^{(d)} = I(X;Y^d)$, for any $d$-view DMC $W^{(d)}$ and input distribution $P_X$.

\begin{lemma}
	\label{lem:concave}
	For any $d$-view DMC $W^{(d)}$ and input distribution $P_X$, we have that $I^{(d)}$ is concave over the positive integers, i.e.,
	\[
	I^{(d)} - I^{(d-1)}\geq I^{(d+1)} - I^{(d)},
	\]
	for all $d\geq 1$.
\end{lemma}
\begin{proof}
	We first rewrite what we intend to prove differently: since $I^{(m)} = H(X) + H(Y^m) - H(X,Y^m)$, for any $m\geq 0$, with $I^{(0)}:= 0$, we would like to show that
	\begin{align}
	H(Y^d) - &H(Y^{d-1})+H(X,Y^{d-1})-H(X,Y^d) \notag\\
	&\geq H(Y^{d+1}) - H(Y^{d})+H(X,Y^{d})-H(X,Y^{d+1}). \label{eq:toshowconcave}
	\end{align}
However, observe that for any $m\geq 0$, $H(X,Y^{m+1})-H(X,Y^{m}) = H(Y_{m+1}|X,Y^m) = H(Y_{m+1}|X)$, by the channel law of $W^{(d)}$. Hence, \eqref{eq:toshowconcave} reduces to showing that
\begin{equation}
H(Y^d) - H(Y^{d-1})\geq H(Y^{d+1}) - H(Y^{d}). \label{eq:toshowconcave2}
\end{equation}
Now, by the submodularity of entropy \cite[Thm. 1.6]{polyanskiywu}, we have that 
\[
H(Y^{d-1},Y_{d+1}) - H(Y^{d-1})\geq H(Y^{d+1}) - H(Y^{d}).
\]
The above implies \eqref{eq:toshowconcave2}, since the distributions of $(Y^{d-1},Y_{d+1})$ and $Y^d$ are equal, by the stationarity of the DMC $W^{(d)}$.
\end{proof}

For clarity, we first write down the capacity $C(\mathsf{Poi}_d(p))$ of the Poisson approximation channel. As argued in Section \ref{sec:main}, the capacity is achieved when the inputs $X\sim P_X = \text{Ber}(1/2)$, yielding
\begin{align}
	&C(\mathsf{Poi}_d(p))\notag\\&= \mathsf{H}(X) - \mathsf{H}(X|R_1,R_2) \notag\\
	&= 1+\sum_{\substack{r_1\geq 0,\\ r_2\geq 0}} \frac{e^{-dp}(dp)^{r_1}}{r_1!}\cdot \frac{e^{-d(1-p)}(d(1-p))^{r_2}}{r_2!}\times \notag\\ &\ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \log \frac{p^{r_1}(1-p)^{r_2}}{p^{r_1}(1-p)^{r_2}+p^{r_2}(1-p)^{r_1}}. \label{eq:poicap}
\end{align}
We now prove Theorem \ref{thm:poibin}.
\begin{proof}
	Consider the mutual information between the input and outputs of the $\mathsf{Poi}_d(p)$ channel when $P_X$ is uniform over the inputs. Since the number of outputs $N=R_1+R_2$ is known to the decoder, we have that
	\begin{align}
		C(\mathsf{Poi}_d(p))&= I(X;R_1,R_2) \notag\\
		&= I(X;R_1,R_2\mid N) \notag \\
		 &= \sum_{n=0}^{\infty}\P[N=n]\cdot I(X;R_1,R_2\mid N=n). \label{eq:poiexp}
	\end{align}
Now, observe that since the sum of a Poi$(dp)$ random variable and a Poi$(d(1-p))$ random variable is distributed according to Poi$(d)$, we have by symmetry that $N\sim \text{Poi}(d)$. Further, it is easy to check that the conditional distribution $P_{R_1,R_2\mid N=n}$ obeys $P_{R_1,R_2\mid N=n}(r_1,r_2\mid n) = \binom{n}{r_1}p^{r_1}(1-p)^{n-r_1}$, for all $r_1,r_2\geq 0$ such that $r_1+r_2 = n$. Hence, we have that $I(X;R_1,R_2\mid N=n) = C(\mathsf{Bin}_n(p))$.

Thus, substituting in \eqref{eq:poiexp}, we get that
\begin{equation}
	\label{eq:expectation}
C(\mathsf{Poi}_d(p)) = \E_{N\sim \text{Poi}(d)}\left[C(\mathsf{Bin}_N(p))\right].
\end{equation}
%	In \eqref{eq:poicap}, for a fixed $r_1, r_2$ in the summation, we introduce the variable $n = r_1+r_2$. The capacity $C(\mathsf{Poi}_d(p))$ can then be rewritten as
%	\begin{align}
%		&C(\mathsf{Poi}_d(p)) \notag\\
%		&= 1+\sum_{n\geq 0}\sum_{r_1=0}^n \frac{e^{-d}d^{n}}{n!}\cdot \binom{n}{r_1}p^{r_1}(1-p)^{n-r_1}\times \notag\\ &\ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \log \frac{p^{r_1}(1-p)^{r_2}}{p^{r_1}(1-p)^{r_2}+p^{r_2}(1-p)^{r_1}} \notag\\
%		&= 1+\sum_{n\geq 0} \frac{e^{-d}d^{n}}{n!}\sum_{r_1=0}^n \binom{n}{r_1}p^{r_1}(1-p)^{n-r_1}\times \notag\\ &\ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \log \frac{p^{r_1}(1-p)^{r_2}}{p^{r_1}(1-p)^{r_2}+p^{r_2}(1-p)^{r_1}} \notag\\
%		&= 1+\sum_{n\geq 0} \frac{e^{-d}d^{n}}{n!}\cdot (C(\mathsf{Bin}_n(p)-1)) = \E_{N\sim \text{Poi}(d)}\left[C(\mathsf{Bin}_N(p))\right].
%	\end{align}
 Next, using the above pleasing expression, we show that $C(\mathsf{Poi}_d(p))$ is indeed a lower bound on $C(\mathsf{Bin}_d(p))$. From Lemma \ref{lem:concave} we have that $C(\mathsf{Bin}_n(p))$ is concave over the positive integers. Therefore, applying Jensen's inequality, we get that
 \begin{align*}
 C(\mathsf{Poi}_d(p)) &= \E_{N\sim \text{Poi}(d)}\left[C(\mathsf{Bin}_N(p))\right]\\
 &\leq C(\mathsf{Bin}_{\E N}(p)) = C(\mathsf{Bin}_{d}(p)).
 \end{align*}
Furthermore, we have that
\begin{align*}
	&C(\mathsf{Bin}_d(p)) - C(\mathsf{Poi}_d(p))\\ &= C(\mathsf{Bin}_d(p)) - \E_{N\sim \text{Poi}(d)}\left[C(\mathsf{Bin}_N(p))\right]\\
	&\leq C(\mathsf{Bin}_d(p))-1+\E_{N\sim \text{Poi}(d)}[Z(p)^N]\\
	&\leq \text{exp}(-d(1-Z(p)))-Z(p)^{2d},
\end{align*}
where the two inequalities make use of Corollary \ref{cor:sasoglu} and the last inequality uses the well-known expression for the moment-generating function of a Poisson random variable.
\end{proof}
\begin{remark}
	For the binomial channel $\overline{\mathsf{Bin}}_n$, whose input is a real number in $[0,1]$, with $n$ output trials, that is considered in \cite{binomialcomposite} too, a suitable Poisson approximation channel $\overline{\mathsf{Poi}}_n$ can be designed. This channel takes as input $X\in [0,1]$ and outputs the pair $(R_1,R_2)$ such that $P_{R_1|X} = \text{Poi}(nX)$ and $P_{R_2|X} = \text{Poi}(n(1-X))$. For $\overline{\mathsf{Poi}}_n$, as above, we will have that  $C(\overline{\mathsf{Poi}}_n) = \E_{N\sim \text{Poi}(n)}\left[C(\overline{\mathsf{Bin}}_N)\right]$. However, the proof of the concavity of the capacity $C(\overline{\mathsf{Bin}}_n)$ as in Lemma \ref{lem:concave} will not hold, owing to the failure of the conditional independence assumption that is crucially employed in the proof. We are hence unable to obtain a lower bound on $C(\overline{\mathsf{Bin}}_n)$ via $C(\overline{\mathsf{Poi}}_n)$.
\end{remark}
